FlameForge: Combustion of Generalized Wooden Structures

We propose a unified volumetric combustion simulator that supports general wooden structures capturing the multi-phase combustion of charring materials. Complex geometric structures can conveniently be represented in a voxel grid for the effective evaluation of volumetric effects. In addition, a signed distance field is introduced to efficiently query the surface information required to compute the insulating effect caused by the char layer. Non-charring materials such as acrylic glass or non-combustible materials such as stone can also be modeled in the simulator. Adaptive data structures are utilized to enable memory-efficient computations within our multiresolution approach. The simulator is qualitatively validated by showcasing the numerical simulation of a variety of scenes covering different kinds of structural configurations and materials. Two-way coupling of our combustion simulator and position-based dynamics is demonstrated capturing characteristic mechanical deformations caused by the combustion process. The volumetric combustion process of wooden structures is further quantitatively assessed by comparing our simulated results to sub-surface measurements of a real-world combustion experiment.

==> 04_method_notes.tex <==
\newpage
\section{Overview}
Basically, this work addresses the combustion simulation for generalized wooden structures beyond trees. To enable this, we extend the combustion model for (cylinders shaped) trees proposed in \cite{pirk2017interactive}. In particular, we convert such general structures (represented as closed triangle mesh) into a Signed Distance Field (SDF), and then the internal distances from the surface are used to control the insulating effect of wood charring in the combustion process. This sdf, together with other fields for fluid simulation (such as velocity, pressure, smoke, temperature, etc.), are implemented with volumetric grids based on OpenVDB. We further explicitly model the volumetric combustion of volatiles and char, which naturally results in a simple unified combustion model for both charring and noncharring solid materials. Extensions along the dimensions of structures and materials enable for a much wider range of potential applications. However, in practice, there still remains a big challenge to make sure that the simulation can resolve the combustion of the thin/sharp structures in an acceptable computational time. To alleviate this, we employed the multiresolution method, where dense grids are used within the local combustion regions, and a sparse grid is used for the global fluid simulation domain.

\section{Fluid and Fire Simulation}

The following are the formulations used in the implementation.
\paragraph{Fluid Dynamics.}
We adopt the Navier-Stokes equation with a nonzero divergence term to enable the volume expansion effect without using a fully compressible model, as in \cite{nielsen2022physics}.

\begin{equation}
\frac{\partial \mathbf{u}} {\partial t} + \mathbf{u}\cdot \nabla \mathbf{u} = -\frac{\nabla p}{\rho} + \nu \nabla^2 \mathbf{u} + \mathbf{f_{buo}}
\label{eq:NS}
\end{equation}

\begin{equation}
\nabla \cdot \mathbf{u} = -  \frac{1}{\rho}\frac{D \rho}{Dt}
\label{eq:divergence}
\end{equation}

where, $p = \tilde{p} - \rho_a \mathbf{g} \cdot \mathbf{z} $ denotes the pressure deviation from the hydrostatic pressure, $\rho_a$ denotes the air density, $\nu$ denotes the kinematic viscosity. 
The buoyancy force acceleration caused by density difference is defined as follows.

%\begin{equation}
%\mathbf{f_{ext} = f_{buo}} 
%\end{equation}

\begin{equation}
\mathbf{f_{buo}}  =  \left(1 - \frac{\rho_a}{\rho}\right)\mathbf{g}
\label{eq:buoyancy}
\end{equation}

The relation between density and temperature is as follows.

\begin{equation}
\rho = \frac{p_{decoupled}}{R_{s} T} \approx \rho_a \frac{T_{amb}}{T}
\end{equation}

%\begin{equation}
%\mathbf{f_{vort}} = \zeta h (\mathbf{N} \times \omega), \omega = \nabla \times \mathbf{u}
%\label{eq:vorticity}
%\end{equation}

%\begin{equation}
%\mathbf{N} = \frac{\mathbf{\eta}}{|\mathbf{\eta|}}, \mathbf{\eta} = \nabla |\mathbf{\omega}|
%\end{equation}

\paragraph{Fire and smoke.} The temperature field evolving process is governed by 

\begin{equation}
\frac{\partial T}{\partial t} + \mathbf{u} \cdot \nabla T = k \nabla^2 T + \gamma_a (T_{amb}^4 - T^4)
\label{eq:atmosphere_heat_transfer}
\end{equation}
$$
\gamma_a = (\varepsilon \sigma A)/(m_aC_{p_a})
$$
where, $k$ denotes the thermal diffusivity, and $\gamma_a$ denotes the radiative cooling coefficient.
According to \cite{tritton2012physical}, $(T_{amb}^4 - T^4)$ is adopted, and the absolute temperature should be used. 

The smoke density is updated according to a passive advection process with a source term produced from the combustion process.

\begin{equation}
\frac{\partial S}{\partial t} + \mathbf{u} \cdot \nabla S = 0
\label{eq:smoke_advec}
\end{equation}

where, $S$ denotes the smoke density field, and $s_S$ is the source term.

\section{Combustion Model}
The combustion model proposed in \cite{pirk2017interactive} was designed for trees (cylindrical shape) and is extended to support general structures and materials in this work. To achieve this goal, we reformulate the combustion model and introduce it in detail in the following aspects.

\paragraph{Volumetric Combustion} In this work, we simulate the combustion process of the materials in a volumetric way, which includes not only the surface temperature, but also the temperature inside the materials. For charring materials (wood, in general cellulosic materials), the materials will be decomposed into volatiles and char via the thermal degradation process (or called pyrolyzing). The combustion of such materials is carried out in two alternative ways involving flaming combustion and smoldering combustion. The flaming combustion is achieved mainly by the high heat released by the volatiles products. However, for the noncharring materials, such as polymethylmethacrylathe (PMMA), the pyrolysis process is confined to the thin melt layer, and no char layers are formed. 
Since the thermal degradation process is very quick compared to the simulation, we adopt the one step global model as shown in \ref{eq:thermal_gradation}, and more details are referred to \cite{di1993modeling}.

\begin{figure}
\centering
\includegraphics[width=0.995\columnwidth]{figures/sdf_diagram.pdf}
\caption{This diagram shows the sdf surfaces (gray dash cures), solid fuel surface (orange curve), and char contraction front (curve in green) and char + volatiles layer (dark gray region), pyrolyzing front surface (dashed orange curve). The left sub-figure show the state before the combustion and the right one shows the state in combustion.}
\label{fig:diagram_cross_section}
\end{figure}

\begin{equation}
%\begin{aligned}
Wood \xrightarrow{\text{Heat}} Volatiles + Char
%\\
%(noncharring)Solid %\xrightarrow{\text{Heat}} Volatiles
%\end{aligned}
\label{eq:thermal_gradation}
\end{equation} 

\begin{equation}
\frac{\partial T_m}{\partial t} = \beta \nabla^2 T_m + \gamma_{w} (T_{amb}^4 - T^4) + s_{T}
\label{eq:solid_combustion}
\end{equation}
$$
\gamma_w = (\varepsilon \sigma A)/(m_wC_{p_w})
$$
\begin{equation}
\frac{\partial S_m}{\partial t} = s_{S}
\label{eq:solid_smoke}
\end{equation}

We define $M, M_v, M_c$ as the mass of solid fuel, volatiles, and char in each voxel cell of the grid. In the thermal degration process, solid fuels are decomposed into volatiles and char, and the mass is in balance, $$M= M_c + M_v$$. For non-charring material, $M_c = 0$. We adopt the discretized formulation for calculating $M_{v, n}, M_{c,n}$ at the $n_{th}$ time step and then the mass loss rate where the negative mass can be easily avoided.

\begin{equation}
M_{v,n} = \max(0, ~M_{v, n-1} - \delta t  \epsilon_v \xi  C)
\label{eq:vol_mass}
\end{equation}

\begin{equation}
M_{c,n} = \max(0, ~M_{c, n-1} - \delta t  \epsilon_c \xi  C)
\label{eq:char_mass}
\end{equation}

Then, the mass loss rates are computed as follows:
\begin{equation}
(\frac{\partial M_v}{\partial t})_n = \frac{M_{v, n} - M_{v, n-1}}{\delta t}
\label{eq:vol_mass_rate}
\end{equation}

\begin{equation}
(\frac{\partial M_c}{\partial t})_n = \frac{M_{c, n} - M_{c, n-1}}{\delta t}
\label{eq:char_mass_rate}
\end{equation}

\begin{equation}
\frac{\partial M}{\partial t} = \frac{\partial M_c}{\partial t} + \frac{\partial M_v}{\partial t}
 %=\frac{\partial (C_v \rho_v + C_c \rho_c)}{\partial t}\delta x \delta y  \delta z
\end{equation}

where, $\delta t, \delta x, \delta y, \delta z$ denotes the temporal and spatial steps, respectively. $\rho_c, \rho_v$ and $M_c, M_v$ are the density and mass of the volatiles and char, $M_c = \rho_c \delta x \delta y  \delta z$, $M_v = \rho_v \delta x \delta y  \delta z$. $\epsilon_c, \epsilon_v, \xi, c$ are the parameters used to jointly control the combustion reaction rate, and will be explained in detail below. In general, $\epsilon_v$ is much larger than $\epsilon_c$ because the combustion of volatiles is much faster than the combustion of char. 

The terms of temperature and smoke source are calculated on the basis of the mass loss rate due to combustion. 
\begin{equation}
s_T = - (T_{M_c}\frac{\partial M_c}{\partial t} + T_{M_v}\frac{\partial M_v}{\partial t})
\label{eq:tem_source}
\end{equation}

\begin{equation}
s_S = - (S_{M_c} \frac{\partial M_c}{\partial t} + S_{M_v} \frac{\partial M_v}{\partial t})
\label{eq:sm_source}
\end{equation}

where, $T_{M_c}, T_{M_v}$ and $S_{M_c}, S_{M_v}$ denote the heat release rate and smoke release rate of the combustion process respectively.

In addition, it is noted that there would also be a drying process before/in the thermal degradation, in which the water content of the materials evaporates. This part is orthogonal to our work and can be easily integrated when necessary even though it is not included in this paper because it is not our focus. 

\paragraph{Temperature Dependent Reaction Rate}  
The temperature dependent reaction rate $\xi$ is a dimensionless parameter whose value range is $\xi\in[0, 1]$. 
\begin{equation}
\xi(T) =  \left \{
\begin{aligned}
    0  & & T<T_{m0} \\
    f((T-T_{m0})/(T_{m1} - T_{m0})) & &
    T_{m0} \leq T \leq T_{m1} \\
    1 & & T>T_{m1} 
\end{aligned}
\right.
\label{eq:rearion_rate}
\end{equation}

where, the sigmoid-like function $f(x) = 3x^2 - 2x^3$ is used to smoothly interpolate from zero to one for the temperatures between the upper and lower temperature limits $T_{m0}$ and $ T_{m1}$. Their values depend on the specific materials. Fox example, for the virgin wood, they can be set $T_{m0} = 150~^{\circ}C, T_{m1} = 450~^{\circ}C$ as used in \cite{pirk2017interactive}. The non-combustible materials can be simulated by setting their lower temperature limits to be infinity.

\paragraph{Char Insulation.}
For the typical charring material, a char layer will be formed in the combustion process. Such a char layer has an insulation effect proportional to its thickness. 
The $C \in [0, 1]$ denotes the dimensionless insulation parameter, defined as follows: 

%which is determined by the distance $h$ to the surface via:

\begin{equation}
C = C_{min} + (1- C_{min})e^{C_rh}
\end{equation}

where, $c_{min}$ denotes the maximum insulation effect with a value in the range of $[0, 1]$.
$C$ is non-linearly proportional to the distance $h$ from the surface of the char layer, $C_r$ denotes the insulation rate due to charring. The distance $h$ is calculated as the absolute value of the signed distance \cite{zhao2005fast} for an inside location of the combustible material.

\paragraph{Char Contraction.} The method for char contraction in \cite{pirk2017interactive} can not be applied to general structures. In our framework, the char contraction phenomenon is explicitly represented as the evolving front of the material mass field $M_c$. The parameter $\epsilon_c$ is used to control the contraction speed. The larger its value is, the char contraction is faster.
  
\paragraph{Heat Exchange.}
The heat exchange between air cell and fuel cell is implemented according to Newton cooling laws: 
\begin{equation}
\frac{\partial T_m}{\partial t} = \phi (T^{neigh} - T_m)
\label{eq:air2solid}
\end{equation}

\begin{equation}
\frac{\partial T}{\partial t} = \phi(T_m^{neigh} - T)
\label{eq:solid2air}
\end{equation}

\begin{equation}
T_{m(i, j, k)}^{neigh} = \frac{L}{D} 
\label{eq:tm_diffusion}
\end{equation}

\begin{equation}
L = 
\begin{aligned}
a_{i-1, j, k}T_{m(i-1, j, k} + a_{i+1, j, k}T_{m(i+1, j, k)} + a_{i, j-1, k}T_{m(i, j-1, k)} \\ 
+ a_{i, j+1, k}T_{m(i, j+1, k)} +  a_{i, j, k-1}T_{m(i, j, k-1)}+ a_{i, j, k+1}T_{m(i, j, k+1)}
\end{aligned}
\end{equation}

\begin{equation}
D = a_{i-1, j, k} + a_{i+1, j, k} + a_{i, j-1, k} + a_{i, j+1, k} + a_{i, j, k+1} + a_{i, j, k-1}
\end{equation}

where, $T_m$ denotes the temperature of the solid materials, and the $a_{i,j}$ denotes the weight for each term; $a_{i,j}=1$ for fuel cell and $a_{i,j}=0$ for the air cell.
where, the average temperature of the neighboring cells is calculated in a similar way as $L/D$ above. Please note the difference in the wights setting. When the average temperature in the neighboured air cells $T^{neigh}$ is calculated, the weight $a_{i,j} = 1$ for air cells, and $a_{i,j} = 0$ for the wood cells. When the average temperature in the neighboured air cells $T^{neigh}_m$ is calculated, the weight $a_{i,j} = 0$ for air cells, and $a_{i,j} = 1$ for the wood cells.

\paragraph{Multiresolution Grids.}
We employed the multiresolution grids method in the simulation, which includes denser grids to resolve the local fine solid structures and a coarse grid for the global fluid simulation domain. The combustion of wooden structures is carried out on the local dense grid. The combustion products (temperature and smoke) are transferred between grids via restriction and prolongation operations in each simulation time step for the overlapped regions. 

\begin{figure}
\centering
\includegraphics[width=0.85\columnwidth]{figures/multi_resolution_grid.pdf}
\caption{This diagram illustrates the multi resolution grids. }
\label{fig:diagram_multi_resolution}
\end{figure}

\begin{table}
\centering \footnotesize
\caption{The summary of all simulation parameters. The values of those parameters above the dashed line are referred from the literature \cite{pirk2017interactive,macleod2023quantifying}. The values of $\epsilon_c$ are calibrated via both numerical and physical experiments. The value of $S_{M_c}, S_{M_v}$ is only for visual effect of smoke. It does not affect the simulation of combustion.}
\label{table:parameter}
\begin{tabular}{c | c | c | c}
%\hline
Name & Description & Value (Range) & Units \\
\hline
$T_{amb}$ & The ambient temperature& 293 & $K$ \\
$\rho_{a}$ & The density of air& 1.2041 & $kgm^{-3}$\\
$\nu$ & The kinematic viscosity of air& 1.6e-5&$m^2s^{-1}$\\
$k$ & Thermal diffusion coefficient of air & 1.8e-5 & $m^2s^{-1}$ \\
$\gamma_a$& Radiative cooling coef. of air & 5.0e-11 & $K^{-3} s^{-1}$ \\
\hdashline
$\phi$ & Heat exchange rate between air and wood & 0.1 &1\\
$\beta$ & Thermal diffusivity (wood) & 0.82e-7 & $m^2s^{-1}$ \\
$\gamma_w$& Radiative cooling coef. of wood & 5.9e-14 & $K^{-3} s^{-1}$ \\
$C_{min}$& The minimum value of $C$ & 0.1 & 1 \\
$C_r$& Rate of insulation & 75.0 & $m^{-1}$ \\
$\epsilon_v$ & Mass loss rate of volatiles & 0.1 & $kgs^{-1}$ \\
$\epsilon_c$ & Mass loss rate of char & [0.1, 1.0]e-3 & $kgs^{-1}$ \\
$T_{M_c}$& Heat generated per unit mass char burned& 3.0e7 & $kg^{-1} K$ \\
$T_{M_v}$& Heat generated per unit mass volatiles burned  & 2.0e7 & $kg^{-1} K$ \\
$T_{m_0}$ & & & \\
\hdashline
$S_{M_c}$ & Smoke per unit mass char & 1.0e3 & $kg^{-1}$\\
$S_{M_v}$ & Smoke per unit mass volatiles & 1.0e3 & $kg^{-1}$\\
\hline
\end{tabular}
\end{table}

\begin{table*}
\centering \footnotesize
\caption{Performance statistics and scene parameters for all simulation results.}
\label{table:performance}
\begin{tabular}{ c | c | c | c | c | c | c | c}
Figures & Scenes & Domain size (m) & $\Delta t$ (s) & Fluid grid size & Fuel grid size ratio & Peak memory & Time per frame \\
\hline
Fig. \ref{xxx} & Wooden boat 
 & $13 \times 6 \times 6$ & 0.033 & $260 \times 120 \times 120$ & 5:1 & 3.3 GB & \\
2 & shape H &&&&&&\\
Fig. \ref{xxx} &Fire in house&&&&&&\\
4 &&&&&&&\\
5 &&&&&&&\\
6 &&&&&&&\\
7 &&&&&&&\\
8 &&&&&&&\\
9 &&&&&&&\\
10 &&&&&&&\\
\hline
\end{tabular}
\end{table*}
